Information Anxiety in Large Language Models

Large Language Models (LLMs) have demonstrated strong performance as knowledge repositories, enabling models to understand user queries and generate accurate and context-aware responses. Extensive evaluation setups have corroborated the positive correlation between the retrieval capability of LLMs and the frequency of entities in their pretraining corpus. We take the investigation further by conducting a comprehensive analysis of the internal reasoning and retrieval mechanisms of LLMs. Our work focuses on three critical dimensions - the impact of entity popularity, the models' sensitivity to lexical variations in query formulation, and the progression of hidden state representations across LLM layers. Our preliminary findings reveal that popular questions facilitate early convergence of internal states toward the correct answer. However, as the popularity of a query increases, retrieved attributes across lexical variations become increasingly dissimilar and less accurate. Interestingly, we find that LLMs struggle to disentangle facts, grounded in distinct relations, from their parametric memory when dealing with highly popular subjects. Through a case study, we explore these latent strains within LLMs when processing highly popular queries, a phenomenon we term information anxiety. The emergence of information anxiety in LLMs underscores the adversarial injection in the form of linguistic variations and calls for a more holistic evaluation of frequently occurring entities.

==> add_info_distance_hidden_llama13b.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/raw/distance_hidden_llama13b.pdf}
\end{figure}

==> add_info_distance_hidden_llama13bchat.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/raw/distance_hidden_llama13bchat.pdf}
\end{figure}

==> add_info_distance_hidden_llama70b.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/raw/distance_hidden_llama70b.pdf}
\end{figure}

==> add_info_distance_hidden_llama7b.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth{figure/raw/distance_hidden_llama7b.pdf}
\end{figure}

==> add_info_distance_hidden_llama7bchat.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/raw/distance_hidden_llama7bchat.pdf}
\end{figure}

==> additional_information_methods_paraphrases_capital.tex <==
\begin{table}[h!]
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.2in}@{\hspace{4em}}p{5.2in}}
\\
\textbf{\texttt{capital}} & 
    \begin{tabular}{l}
        What is the \format{capital} of <MASK>?\\
        What is the \format{primary city} in <MASK>?\\
        Which \format{urban center} holds a \format{central role} in <MASK>?\\
        Which city \format{houses the main government} of <MASK>?\\
        What city is the \format{main administrative center} of <MASK>?\\
        What \format{urban area} holds the \format{capital status} of <MASK>?\\
        Which city is the \format{political focal point} of <MASK>?\\
        Which city is the \format{primary seat of authority} for <MASK>?\\
        What is the \format{principal city} of <MASK>?\\
        What is the \format{chief city} of <MASK>?\\
    \end{tabular}\\
\end{tabular}
}
\end{table}


==> additional_information_methods_paraphrases_genre.tex <==
\begin{table}[h!]
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.2in}@{\hspace{4em}}p{5.2in}}
\\
\textbf{\texttt{genre}} & \begin{tabular}{l}
        What \format{category} does <MASK> belong to?\\
        What \format{kind of classification} does <MASK> fall under?\\
        What \format{type} does <MASK> fall under?\\
        What \format{group} does <MASK> fall under?\\
        What \format{kind} does <MASK> fall under?\\
        What \format{class} does <MASK> fall under?\\
        What \format{style} can <MASK> be categorized into?\\
        Which \format{division} does <MASK> come under?\\
        In what \format{bracket} does <MASK> reside?\\
        What \format{domain} does  <MASK> fit within?\\
\end{tabular}\\
\bottomrule
\end{tabular}
}
\end{table}




==> additional_information_methods_paraphrases_occupation.tex <==
\begin{table}[h!]
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.2in}@{\hspace{4em}}p{5.2in}}
\\
\textbf{\texttt{occupation}} & \begin{tabular}{l}
    What does <MASK> do for a \format{living}?\\
    What is <MASK>'s \format{occupation}?\\
    What is <MASK>'s \format{profession}?\\
    What is <MASK>'s \format{line of work}?\\
    What \format{job role} is <MASK> engaged in?\\
    What \format{career path} has <MASK> chosen?\\
    What \format{field of employment} is <MASK> part of?\\
    What is <MASK>'s source of \format{professional engagement}?\\
    What is <MASK>'s \format{vocational pursuit}?\\
    What \format{field of work} is <MASK> engaged in?\\
\end{tabular}\\
\\
\end{tabular}
}
\end{table}

==> additional_information_methods_paraphrases_religion.tex <==
\begin{table}[h!]
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.2in}@{\hspace{4em}}p{5.2in}}
\\
\textbf{\texttt{religion}} & \begin{tabular}{l}

        What is the \format{religion} of <MASK>?\\
        What \format{faith} does <MASK> follow?\\
        What is the \format{religious affiliation} of <MASK>?\\
        Which \format{religious doctrine} does <MASK> subscribe to?\\
        What \format{theology} is <MASK> aligned with?\\
        What is the \format{religious identity} of <MASK>?\\
        What \format{belief system} does <MASK> ascribe to?\\
        What \format{religious school of thought} does <MASK> follow?\\
        What is <MASK>'s \format{spirituality}?\\
        What is the \format{religious allegiance} of <MASK>?\\

\end{tabular}\\
\end{tabular}
}
\end{table}


==> additional_information_methods_paraphrases_screenwriter.tex <==
\begin{table}[h!]
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.2in}@{\hspace{4em}}p{5.2in}}
\\
\\
\textbf{\texttt{screenwriter}} & \begin{tabular}{l}
        Who was the \format{screenwriter} for <MASK>?\\
        Who \format{wrote the screenplay} for <MASK>?\\
        Who was the \format{scribe of the screenplay} in <MASK>?\\
        Who took on the \format{role of crafting} <MASK>'s \format{script}?\\
        Who was responsible for \format{composing the screenplay} of <MASK>?\\
        Who was the \format{wordsmith behind the screenplay} of <MASK>?\\
        Who \format{penned the script} for <MASK>?\\
        Who \format{authored the screenplay} of <MASK>?\\
        Who was the primary influencer in shaping <MASK>'s \format{screenplay composition}?\\
        Who \format{scripted} <MASK>'s story?\\
\end{tabular}\\
\\
\end{tabular}
}
\end{table}


==> additional_information_methods_paraphrases_sport.tex <==
\begin{table}[h!]
\setlength{\tabcolsep}{2pt} % Adjusting column separation
\renewcommand{\arraystretch}{1.0} % Reducing cell padding
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1.2in}@{\hspace{4em}}p{5.2in}}
\\
\textbf{\texttt{sport}} & \begin{tabular}{l}
        What \format{sport} does <MASK> play?\\
        What \format{athletic activity} does <MASK> participate in?\\
        What \format{game} does <MASK> compete in?\\
        What \format{field of sports} is <MASK> involved with?\\
        Which \format{athletic endeavour} does <MASK> pursue?\\
        What \format{physical activity} does <MASK> perform as a sport?\\
        What \format{recreational sport} does <MASK> enjoy?\\
        What \format{sport} does <MASK> enjoy playing?\\
        What \format{professional sport} does <MASK> play?\\
        What \format{game} does <MASK> actively participate in?\\
\end{tabular}\\
\bottomrule
\end{tabular}
}
\end{table}

